Construction of 'Support Vector' Machine Feature Spaces via Deformed Weyl-Heisenberg Algebra

This paper uses deformed coherent states, based on a deformed Weyl-Heisenberg algebra that unifies the well-known SU(2), Weyl-Heisenberg, and SU(1,1) groups, through a common parameter. We show that deformed coherent states provide the theoretical foundation of a meta-kernel function, that is a kernel which in turn defines kernel functions. Kernel functions drive developments in the field of machine learning and the meta-kernel function presented in this paper opens new theoretical avenues for the definition and exploration of kernel functions. The meta-kernel function applies associated revolution surfaces as feature spaces identified with non-linear coherent states. An empirical investigation compares the deformed SU(2) and SU(1,1) kernels derived from the meta-kernel which shows performance similar to the Radial Basis kernel, and offers new insights (based on the deformed Weyl-Heisenberg algebra).

==> apssamp.tex <==
@inproceedings{boser1992training,
  title={A training algorithm for optimal margin classifiers},
  author={Boser, Bernhard E and Guyon, Isabelle M and Vapnik, Vladimir N},
  booktitle={Proceedings of the fifth annual workshop on Computational learning theory},
  pages={144--152},
  year={1992},
  organization={ACM}
}
@inproceedings{schiilkop1995extracting,
  title={Extracting support data for a given task},
  author={Sch\"{o}lkopf, PB and Burgest, Chris and Vapnik, Vladimir},
  booktitle={Proceedings of the 1st international conference on knowledge discovery \& data mining},
  pages={252--257},
  year={1995}
}

@article{claesen2014easy,
  title={Easy hyperparameter search using optunity},
  author={Claesen, Marc and Simm, Jaak and Popovic, Dusan and Moreau, Yves and De Moor, Bart},
  journal={arXiv preprint arXiv:1412.1114},
  year={2014}
}

@article{scikit-learn,
 title={Scikit-learn: Machine Learning in {P}ython},
 author={Pedregosa, F. and Varoquaux, G. and Gramfort, A. and Michel, V.
         and Thirion, B. and Grisel, O. and Blondel, M. and Prettenhofer, P.
         and Weiss, R. and Dubourg, V. and Vanderplas, J. and Passos, A. and
         Cournapeau, D. and Brucher, M. and Perrot, M. and Duchesnay, E.},
 journal={Journal of Machine Learning Research},
 volume={12},
 pages={2825--2830},
 year={2011}
}

@article{stone1974cross,
  title={Cross-validatory choice and assessment of statistical predictions},
  author={Stone, Mervyn},
  journal={Journal of the Royal Statistical Society: Series B (Methodological)},
  volume={36},
  number={2},
  pages={111--133},
  year={1974},
  publisher={Wiley Online Library}
}

@misc{Charles2013,
  author = {Brandl, G. et al},
  title = {Python Object Serialization},
  year = {2019},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/python/cpython/blob/3.7/Doc/library/pickle.rst}},
  commit = {ff2a5c0204bd08cde2f2c10605e1f9b442b5a7d6}
}

@misc{daly_daly_2019, 
    title={Amazon Web Services Elastic-Compute 2}, howpublished={https://docs.aws.amazon.com/ec2/index.html}, 
    publisher={CGA Canada Publications}, 
    author={Amazon Web Services},
    year={2019}}

@inproceedings{osuna1998reducing,
  title={Reducing the run-time complexity of support vector machines},
  author={Osuna, Edgar and Girosi, Federico},
  booktitle={International Conference on Pattern Recognition (submitted)},
  year={1998}
}

@inproceedings{gretton2001support,
  title={Support vector regression for black-box system identification},
  author={Gretton, Arthur and Doucet, Arnaud and Herbrich, Ralf and Rayner, Peter JW and Scholkopf, Bernhard},
  booktitle={Proceedings of the 11th IEEE Signal Processing Workshop on Statistical Signal Processing (Cat. No. 01TH8563)},
  pages={341--344},
  year={2001},
  organization={IEEE}
}

@article{schuld2019quantum,
  title={Quantum machine learning in feature Hilbert spaces},
  author={Schuld, Maria and Killoran, Nathan},
  journal={Physical review letters},
  volume={122},
  number={4},
  pages={040504},
  year={2019},
  publisher={APS}
}

@article{havlivcek2019supervised,
  title={Supervised learning with quantum-enhanced feature spaces},
  author={Havl{\'\i}{\v{c}}ek, Vojt{\v{e}}ch and C{\'o}rcoles, Antonio D and Temme, Kristan and Harrow, Aram W and Kandala, Abhinav and Chow, Jerry M and Gambetta, Jay M},
  journal={Nature},
  volume={567},
  number={7747},
  pages={209},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{faulhuber2018gaussian,
  title={Gaussian distributions and phase space Weyl--Heisenberg frames},
  author={Faulhuber, Markus and de Gosson, Maurice A and Rottensteiner, David},
  journal={Applied and Computational Harmonic Analysis},
  year={2018},
  publisher={Elsevier}
}

@article{castillo2019polynomial,
  title={Polynomial Heisenberg algebras, multiphoton coherent states and geometric phases},
  author={Castillo-Celeita, Miguel and Bautista, Erik Diaz and Fernandez, David J},
  journal={Physica Scripta},
  year={2019},
  publisher={IOP Publishing}
}

@article{dehdashti2013coherent,
  title={COHERENT STATE OF $\alpha$-DEFORMED WEYL--HEISENBERG ALGEBRA},
  author={Dehdashti, Sh and Mahdifar, A and Roknizadeh, R},
  journal={International Journal of Geometric Methods in Modern Physics},
  volume={10},
  number={05},
  pages={1350014},
  year={2013},
  publisher={World Scientific}
}

@article{dehdashti2015realization,
  title={Realization of non-linear coherent states by photonic lattices},
  author={Dehdashti, Shahram and Li, Rujiang and Liu, Jiarui and Yu, Faxin and Chen, Hongsheng},
  journal={AIP Advances},
  volume={5},
  number={6},
  pages={067165},
  year={2015},
  publisher={AIP Publishing}
}

@inproceedings{chapelle2005semi,
  title={Semi-supervised classification by low density separation.},
  author={Chapelle, Olivier and Zien, Alexander},
  booktitle={AISTATS},
  volume={2005},
  pages={57--64},
  year={2005},
  organization={Citeseer}
}

@article{carinena2005central,
  title={Central potentials on spaces of constant curvature: The Kepler problem on the two-dimensional sphere S 2 and the hyperbolic plane H 2},
  author={Cari{\~n}ena, Jos{\'e} F and Ra{\~n}ada, Manuel F and Santander, Mariano},
  journal={Journal of Mathematical Physics},
  volume={46},
  number={5},
  pages={052702},
  year={2005},
  publisher={AIP}
}

@book{combescure2012coherent,
  title={Coherent states and applications in mathematical physics},
  author={Combescure, Monique and Robert, Didier},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{Haykin08,
  title={Neural Networks and Learning Machines: A Comprehensive Foundation},
  author={Simon O. Haykin},
  year={2008},
  publisher={Pearson (3rd edition)}
}

@book{ali2000coherent,
  title={Coherent states, wavelets and their generalizations},
  author={Ali, Syed Twareque and Antoine, Jean-Pierre and Gazeau, Jean-Pierre and others},
  volume={3},
  year={2000},
  publisher={Springer}
}


@book{bengtsson2017geometry,
  title={Geometry of quantum states: an introduction to quantum entanglement},
  author={Bengtsson, Ingemar and {\.Z}yczkowski, Karol},
  year={2017},
  publisher={Cambridge university press}
}

@article{cortes1995support,
  title={Support-vector networks},
  author={Cortes, Corinna and Vapnik, Vladimir},
  journal={Machine learning},
  volume={20},
  number={3},
  pages={273--297},
  year={1995},
  publisher={Springer}
}




@article{rebentrost2014quantum,
  title={Quantum support vector machine for big data classification},
  author={Rebentrost, Patrick and Mohseni, Masoud and Lloyd, Seth},
  journal={Physical review letters},
  volume={113},
  number={13},
  pages={130503},
  year={2014},
  publisher={APS}
}

@article{pitowsky1994george,
  title={George Boole's ‘conditions of possible experience’and the quantum puzzle},
  author={Pitowsky, Itamar},
  journal={The British Journal for the Philosophy of Science},
  volume={45},
  number={1},
  pages={95--125},
  year={1994},
  publisher={Oxford University Press}
}

@article{goh2018geometry,
  title={Geometry of the set of quantum correlations},
  author={Goh, Koon Tong and Kaniewski, J{\k{e}}drzej and Wolfe, Elie and V{\'e}rtesi, Tam{\'a}s and Wu, Xingyao and Cai, Yu and Liang, Yeong-Cherng and Scarani, Valerio},
  journal={Physical Review A},
  volume={97},
  number={2},
  pages={022104},
  year={2018},
  publisher={APS}
}

@article{vourdas2019probabilistic,
  title={Probabilistic inequalities and measurements in bipartite systems},
  author={Vourdas, Apostol},
  journal={Journal of Physics A: Mathematical and Theoretical},
  year={2019},
  publisher={IOP Publishing}
}

@article{mehta2019high,
  title={A high-bias, low-variance introduction to machine learning for physicists},
  author={Mehta, Pankaj and Bukov, Marin and Wang, Ching-Hao and Day, Alexandre GR and Richardson, Clint and Fisher, Charles K and Schwab, David J},
  journal={Physics reports},
  year={2019},
  publisher={Elsevier}
}

@article{killoran2019strawberry,
  title={Strawberry fields: A software platform for photonic quantum computing},
  author={Killoran, Nathan and Izaac, Josh and Quesada, Nicol{\'a}s and Bergholm, Ville and Amy, Matthew and Weedbrook, Christian},
  journal={Quantum},
  volume={3},
  pages={129},
  year={2019},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}

@article{killoran2018continuous,
  title={Continuous-variable quantum neural networks},
  author={Killoran, Nathan and Bromley, Thomas R and Arrazola, Juan Miguel and Schuld, Maria and Quesada, Nicol{\'a}s and Lloyd, Seth},
  journal={arXiv preprint arXiv:1806.06871},
  year={2018}
}

@article{steinbrecher2019quantum,
  title={Quantum optical neural networks},
  author={Steinbrecher, Gregory R and Olson, Jonathan P and Englund, Dirk and Carolan, Jacques},
  journal={npj Quantum Information},
  volume={5},
  number={1},
  pages={60},
  year={2019},
  publisher={Nature Publishing Group}
}

@inproceedings{srinivasan2018learning,
  title={Learning and inference in hilbert space with quantum graphical models},
  author={Srinivasan, Siddarth and Downey, Carlton and Boots, Byron},
  booktitle={Advances in Neural Information Processing Systems},
  pages={10338--10347},
  year={2018}
}

@inproceedings{Bhattacharyya11,
  title={Performance Analysis of Left/Right Hand Movement Classification from EEG Signal by Intelligent Algorithms },
  author={Saugat Bhattacharyya, Anwesha Khasnobish, Amit Konar, D.N Tibarewala, Atulya K. Nagar},
  booktitle={IEEE Symposium on Computational Intelligence, Cognitive Algorithms, Mind, and Brain (CCMB)},
  pages={1--8},
  year={2011}
}

@article{Ali06,
    title={A meta-learning approach to automatic kernel selection for support vector machines},
    author={Shawkat Ali and Kate A.Smith-Miles},
    journal={Neurocomputing},
    year={2006},
    volume={70},
    pages={173--186}
}


@article{adhikary2019supervised,
  title={Supervised learning with a quantum classifier using a multi-level system},
  author={Adhikary, Soumik and Dangwal, Siddharth and Bhowmik, Debanjan},
  journal={arXiv preprint arXiv:1908.08385},
  year={2019}
}

@article{bartkiewicz2019experimental,
  title={Experimental kernel-based quantum machine learning in finite feature space},
  author={Bartkiewicz, Karol and Gneiting, Clemens and {\v{C}}ernoch, Anton{\'\i}n and Jir{\'a}kov{\'a}, Kate{\v{r}}ina and Lemr, Karel and Nori, Franco},
  journal={arXiv preprint arXiv:1906.04137},
  year={2019}
}

@misc{schuld2019machine,
  title={Machine learning in quantum spaces},
  author={Schuld, Maria},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{kubler2019quantum,
  title={Quantum mean embedding of probability distributions},
  author={K{\"u}bler, Jonas M and Muandet, Krikamol and Sch{\"o}lkopf, Bernhard},
  journal={Physical Review Research},
  volume={1},
  number={3},
  pages={033159},
  year={2019},
  publisher={APS}
}
